3BASiL: An Algorithmic Framework for Sparse plus Low-Rank Compression of LLMs

Sparse plus Low-Rank $(\mathbf{S} + \mathbf{LR})$ decomposition of Large Language Models (LLMs) has emerged as a promising direction in model compression, aiming to decompose pre-trained model weights into a sum of sparse and low-rank matrices $(\mathbf{W} \approx \mathbf{S} + \mathbf{LR})$. Despite recent progress, existing methods often suffer from substantial performance degradation compared to dense models. In this work, we introduce 3BASiL-TM, an efficient one-shot post-training method for $(\mathbf{S} + \mathbf{LR})$ decomposition of LLMs that addresses this gap. Our approach first introduces a novel 3-Block Alternating Direction Method of Multipliers (ADMM) method, termed 3BASiL, to minimize the layer-wise reconstruction error with convergence guarantees. We then design an efficient transformer-matching (TM) refinement step that jointly optimizes the sparse and low-rank components across transformer layers. This step minimizes a novel memory-efficient loss that aligns outputs at the transformer level. Notably, the TM procedure is universal as it can enhance any $(\mathbf{S} + \mathbf{LR})$ decomposition, including pure sparsity. Our numerical experiments show that 3BASiL-TM reduces the WikiText2 perplexity gap relative to dense LLaMA-8B model by over 30% under a (2:4 Sparse + 64 LR) configuration, compared to prior methods. Moreover, our method achieves over 2.5x faster compression runtime on an A100 GPU compared to SOTA $(\mathbf{S} + \mathbf{LR})$ method. Our code is available at https://github.com/mazumder-lab/3BASiL.

==> Tex/sec-algorithm.tex <==
% !TEX root = ../main.tex


% \begin{algorithm}
% \caption{\loraft\ourmethodplus}
% \label{alg:3basil}
% \begin{algorithmic}[1]
% \Statex \textbf{Input:} Pre-trained LLM with $\{T_i\}_{i=1}^T$ transformer blocks, each contains $\{\bfW^{(i,\ell)}\}_{\ell = 1}^L$ layers, calibration data $\bfX$, target sparsity $\mathcal{S}$, target rank $r$, initial quadratic penalty term $\rho > 0$, Hessian regularization term $\lambda$.
% \Statex \textbf{Output:}  Compressed model with $\{\bfS^{(i,\ell)}, \bfL^{(i,\ell)}\}, i \in {T}, \ell \in [L]$.

% \vspace{0.5em}
% \For{each transformer block $T_i$ in the LLM}
%     \Statex \quad\; \textbf{Step 1: \ourmethod layer-wise \slr decomposition (Required)}
%     \For{each layer $\ell$ in $T_i$}
%         \State $\bfH = \left(\bfX^{(i,\ell)}\right)^\top \bfX^{(i,\ell)} + \lambda$, where $\bfX^{(i,\ell)}$ are outputs of previous layer.
%         \begin{align*}
%             \min_{\bfS^{(i,\ell)}, \bfL^{(i,\ell)}} \|\bfX^{(i,\ell)} \bfW^{(i,\ell)} - \bfX^{(i,\ell)}(\bfS^{(i,\ell)} + \bfL^{(i,\ell)})\|_F^2\\
%             \text{s.t. } \bfS^{(i,\ell)} \in \mathcal{S}^{(i,\ell)}, \text{rank}(\bfL^{(i,\ell)}) \leq r
%         \end{align*}
%         \State Replace $\bfW^{(i,\ell)}$ with $\bfS^{(i,\ell)} + \bfL^{(i,\ell)}$ for subsequent layers
%     \EndFor
% \EndFor

% \vspace{0.5em}
% \Statex \textbf{Step 2: Transformer-level Matching (Optional)}
% \For{each transformer block $T_i$ in the LLM}
%     \State Collect input-output pairs $(X_i, Y_i)$ using calibration data
%     \State Refine sparse components by solving:
%     \begin{align*}
%         \min_{\{\bfS^{(i,\ell)}\}_{\ell}} \|T_i(X_i; \{\bfW^{(i,\ell)}\}) - T_i(X_i; \{\bfS^{(i,\ell)} + \bfL^{(i,\ell)}\})\|_F^2
%     \end{align*}
%     \State Update $\bfS^{(i,\ell)}$ for all layers in $T_i$
% \EndFor

% \vspace{0.5em}
% \Statex \textbf{Step 3: Task-specific LoRA Fine-tuning (Optional)}
% \State Freeze sparse components $\{\bfS^{(i,\ell)}\}$ .
% \State Fine-tune low-rank components $\{\bfL^{(i,\ell)}\}$ on downstream task using LoRA framework.

% \State \Return compressed model with $\{\bfS^{(i,\ell)}, \bfL^{(i,\ell)}\}, i \in {T}, \ell \in [L]$.
% \end{algorithmic}
% \end{algorithm}



